Coplanar Repeats by Energy Minimization

This paper proposes an automated method to detect, group and rectify arbitrarily-arranged coplanar repeated elements via energy minimization. The proposed energy functional combines several features that model how planes with coplanar repeats are projected into images and captures global interactions between different coplanar repeat groups and scene planes. An inference framework based on a recent variant of $\alpha$-expansion is described and fast convergence is demonstrated. We compare the proposed method to two widely-used geometric multi-model fitting methods using a new dataset of annotated images containing multiple scene planes with coplanar repeats in varied arrangements. The evaluation shows a significant improvement in the accuracy of rectifications computed from coplanar repeats detected with the proposed method versus those detected with the baseline methods.

==> algorithm_block.tex <==
\setlength{\interspacetitleruled}{0pt}
\setlength{\algotitleheightrule}{0pt}
\begin{algorithm}
  \caption{Coplanar repeats by energy minimization
    \label{alg:energy}}
  \begin{algorithmic}[1]
    \Function{Repeats}{$\meas, \ve[w]$}
      \State{$\ve[w] \gets \text{tuned weight vector}$}
      \State{$\hat{\beta}  \gets \text{Propose} (\meas)$}
      \Repeat 
        \State{$\hat{\ve[y]} \gets \argmin_{\ve[y]}\,\ve[w]^{\T}\psi(\meas,\lblg,\beta(\ve[y])=\hat{\beta})$}
        \State{$\hat{\beta} \gets \argmin_{\beta}\,\ve[w]^{\T}\psi(\meas,\lblg=\hat{\lblg},\beta(\hat{\lblg}))$} 
        \State{$E \ \gets  \ \ve[w]^{\T} \psi(\meas, \hat{\ve[y]}, \hat{\beta})$}
      \Until{$\frac{\Delta E}{|E|} > \epsilon$ }

      \State \Return{$\hat{\ve[y]}$}
    \EndFunction
  \end{algorithmic}
\end{algorithm}


==> contributions.tex <==
%
%
%balances the
%appearance amd geometric similarity of repeats with their geometric
%consistency to consrtaints induced by their underlying scene plane.
%
%
%of repeats as well as their
%consistency 
%underlying scene plane.
%
%
% automated method to detect repeats,
%rectify their underlying scene planes and a
%
%
% global energy model that balances the
%geometry and appearance of multiple scene planes, coplanar repeats, 
%
% Only recent
%innovations in energy minimization and learning have enabled the
%incorporation of the needed higher-order terms into a fast inference
%problem, and the learning of weights for energy functionals
%(equivalently discriminant functions) with structured outputs.
%
%The proposed automated method formulates imaged
%coplanar repeated scene-element grouping, scene-plane vanishing line
%estimation and image segmentation as a joint energy minimization
%problem. The energy function globally models the scene and the scene
% labeling problem
%formulated with a \emph{global} energy functione. Extracted local textured image
%patches, called distinguished regions, are grouped so that members
%represent the same underlying repeating coplanar scene element.
%
%
%Repeat grouping is an ill-posed problem: Given the number of
%distinguished regions extracted and their feature noise, by chance,
%some features will closely match incorrect global models. Visual
%ycoherence is encouraged through pairwise interactions of
%distinguished region texture descriptors. The extracted features
%include superpixels that over-segment the image into visually
%homogeneous patches. The superpixels are used to define the feature
%interactions of a regularization term that encourages overlapping
%superpixels and distinguished regions to take on labels that are
%consistent with a common underlying scene plane. This construction
%enables distinguished regions on the periphery of large homogeneous
%regions (which are common on scene planes) to interact while
%preserving discontinuity across imaged edges that commonly occur at
%scene plane intersections (\eg, at building corners) where there are
%usually dense patches of distinguished regions. This domain specific
%interaction is not possible with strictly pairwise interactions of
%distinguished regions using, \eg, a fixed radius or k-nearest
%neighbors to define interaction neighborhoods.
%
% Each extracted distinguished region is
%assigned a label corresponding to a repeat grouping, which is defined
%as a set of distinguished regions that jointly satisfy single-view
%geometric constraints and have a mutual affinity for the group's
%appearance representation. In addition, over-segmented image regions
%called superpixels are labeled with vanishing lines that are
%consistent with their underlying scene planes, giving a useful
%partitioning of the scene (\eg, separating building facades and
%clutter).  The proposed method is fully automated, fast, and works
%reliably on a very wide class of images with arbitrarily arranged
%patterns on unknown numbers of scene planes in the presence of
%surrounding clutter and occlusions.
%
%
%Detecting coplanar repeats is a chicken-and-egg problem: scene
%geometries and tentative repeat groupings are needed to measure the
%cost of a labeling, but these quantities are apriori unknown. An
%additional challenge is that estimation of real-valued outputs, such
%as scene plane vanishing lines, are not easily incorporated into
%inference for discretely labeled energies. To address both issues,
%minimization of the global energy proceeds by block-coordinate descent
%in a manner similar to \cite{Isack-IJCV12}: Scene geometries are
%sampled and repeat groupings consistent with sampled geometries are
%proposed as labels. Then the descent loop alternates from the labeling
%of distinguished regions and superpixels to the estimation of scene
%geometry and repeat group appearance representation until
%convergence. A recent variant of $\alpha$-expansion
%\cite{Delong-IJCV12} is used for labeling since it is relatively fast,
%provides an error bound, and accommodates regularization terms that
%penalize for over-fitting.
%
%Rigorous performance evaluations in the repeat grouping literature are
%conspicuously missing, so there are no appropriate truthed datasets or
%standard loss functions available, each of which is also needed to
%learn the weights of the proposed energy function. We introduce a new
%dataset that provides labeling truth for a challenging set of 70
%images, and a tractable loss function that effectively characterizes
%bad labelings.
%
% Spatial regularization is achieved
%through distinguished region-to-superpixel interactions and
%inter-superpixel interactions; in other words, the superpixels act as
%a connective structure between disparate distinguished regions. This
%hybrid strategy of using sparse and dense features enables local and
%global regularization with the use of only pairwise interactions,
%which simplifies the proposed inference algorithm. An additional
%benefit of including superpixels is that the image can be segmented at
%pixel level into planar and non-planar regions.
%
%
%
%
%
%\ie, homogeneous
%image patches will have few or no regions extracted, which This phenomenon
%poses a challenge for
%
% which
%motivates the inclusion of multiple geometric and appearance affinity
%costs and regularization costs that model labeling correlations and
%penalize for scene complexity.
%
%
%Thus regularization is required to ensure Labeling is regularized by The CRF is used to
%incorporate multiple geometric and photometric constraints, to
%regularize the grouping of local features into repeats based on the
%features' spatial layout and similarity in appearance, and to control
%scene complexity\ (\ie the numbers of lines at infinity and repeat
%groupings present in the image). Geometric constraints are enforced
%globally, \eg, repeats on parallel scene planes jointly participate in
%geometry and appearance model estimation.
%
%
% in which an
%optimal labeling groups distinguished regoins and 
%
%
% the proposed method is \emph{unified
%framework} for balancing 
%
%
%t are justified by sc
%considerations specific to repeat grouping.
%
%
%This amotivates the
%formulation of a global energy functional that simultaneously
%evaluates multiple constraints while regularizing labeling by
%incorporating priors or correlations that can be justified by
%real-world constraints specific to repeat grouping (\eg, a term
%encouraging spatial coherence of features that share the same
%vanishing line is justified since close-by features likely lie on the
%same scene plane). are either not fully-automated, not general enough,
%or not sufficiently robust for use on large-scale databases;
%respectively, they assume the presence of user annotations
%\cite{Zhang-IJCV12} or specific scene structure (\eg, orthogonal sets
%of parallel scene lines) or a dominant scene plane
%\cite{Aiger-EG12,Zhang-IJCV12}, or use a greedy approach for coplanar
%repeat detection that typically takes the form of an estimation
%pipeline in which constraints are applied sequentially at different
%algorithm stages
%
%
%Renewed interest in coplanar repeat grouping is motivated by recent
%image-retrieval, geo-location and 3D-reconstruction attempts on
%large-scale image databases of urban centers where coplanar repeated
%patterns are ubiquitous
%\cite{Sattler-ECCV12,Schoenberger-CVPR15,Torii-CVPR13}. Repeated
%patterns are known to violate statistical independence assumptions
%frequently made in conventional retrieval and reconstruction
%approaches. There have been some attempts to account for skewed
%similarity statistics caused by repetitive patterns, \eg, Jegou, Shi
%\etal \cite{Jegou-CVPR09,Shi-CVPR15}, but repetitive patterns remain
%problematic for many computer vision tasks even though their rich
%structure should provide significant performance benefits. So there is
%a need for a method that can robustly group and model repeats on
%varied scene content in large image databases.
%
%
%
%or{red}{write some stuff about advances in energy  minimization}
%
%{Contributions}

%
%rouping is cast as probabilistic inference on a conditional
%ield (CRF), where hidden states correspond to feature grouping
%es. The CRF is used to incorporate multiple geometric and
%ric constraints, to regularize the grouping of local features
%eats based on the features' spatial layout and similarity in
%ce, and to control scene complexity\ (\ie the numbers of lines
%ity and repeat groupings present in the image). Geometric
%nts are enforced globally, \eg, repeats on parallel scene
%ointly participate in geometry and appearance model estimation.
% repeats are identified by CRF labeling. We also distinguish
%nd non-planar singletons (considered outliers in this context
%ey are non-repeating), which also helps regularize repeat
% and can subsequently be used, \eg, to segment buildings from
%dings in urban settings. Critically, scene priors and
%ty penalties (\ie, pairwise and higher-order CRF potentials,
%vely) are designed so that fast labeling is possible by
%e with $\alpha$-expansion.
%
%epetitive patterns are affected locally by varied lighting
%ns and occlusions and globally by perspective
%ion. These factors motivate a bottom-up approach in which
%ished regions (\ie local image patches of high texture) are
%d and then grouped if their pre-images correspond to coplanar
% scene elements.
%
%regularity is more difficult to accomplish since the
%tion of distinguished regions depends on the underlying
%texture/ To address this, the image is segmented into
%ous regions known as superpixels. Spatial regularization is
% indirectly through distinguished region-to-superpixel
%ions and inter-superpixel interactions; in other words, the
%els act as a connective structure between disparate
%ished regions. This hybrid strategy of using sparse and dense
% enables local and global regularization with the use of only
% interactions, which simplifies the proposed inference
%m. An additional benefit of including superpixels is that the
%n be segmented at pixel level into planar and non-planar
%7


==> defs.tex <==
\DeclareMathOperator{\median}{median} 

\newcommand{\BigO}[1]{\ensuremath{\operatorname{O}\bigl(#1\bigr)}}
\newcommand{\suchthat}{\;\ifnum\currentgrouptype=16 \middle\fi|\;}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

\newcommand*\mean[1]{\bar{#1}}

% RANSAC
\newcommand{\RANSAC}{\textsc{ransac}\xspace}
\newcommand{\MLESAC}{\textsc{mlesac}\xspace}
\newcommand{\RRANSAC}{\textsc{r-ransac}\xspace}
\newcommand{\rr}{\textsc{r-ransac}\xspace}
\newcommand{\NAPSAC}{\textsc{napsac}\xspace}
\newcommand{\LORANSAC}{\textsc{lo-ransac}\xspace}
\newcommand{\MINPRAN}{\textsc{minpran}\xspace}
\newcommand{\ransac}{\RANSAC}
\newcommand{\prosac}{\textsc{prosac}\xspace}
\newcommand{\LO}{\textsc{lo}\xspace}
\newcommand{\DEGEN}{\textsc{degensac}\xspace}
\newcommand{\degen}{\textsc{degensac}\xspace}
\newcommand{\PLUNDER}{\textsc{plunder}\xspace}

% SotA
\newcommand{\sift}{SIFT\xspace}
\newcommand{\sifts}{SIFTs\xspace}
\newcommand{\laf}{LAF\xspace}
\newcommand{\lafs}{LAFs\xspace}
\newcommand{\mser}{MSER\xspace}
\newcommand{\mserp}{MSER+\xspace}
\newcommand{\mserm}{MSER-\xspace}
\newcommand{\msers}{MSERs\xspace}
\newcommand{\dr}{DR\xspace}
\newcommand{\drs}{DRs\xspace}
\newcommand{\rootsift}{RootSIFT\xspace}
\newcommand{\rootsifts}{RootSIFTs\xspace}

% vectors & matrices
\newcommand{\inv}{{-1}}
\newcommand{\ma}[1]{\ensuremath{\mathtt{#1}}\xspace}
\newcommand{\Hg}{\ensuremath{\ma{H}}\xspace}
\newcommand{\Hinf}{\ensuremath{\ma{H}_{\infty}}\xspace}
\newcommand{\estHg}{\ensuremath{\ma{\hat{H}}}\xspace}
\newcommand{\estHinf}{\ensuremath{\ma{\hat{H}_{\infty}}}\xspace}
\newcommand{\Fm}{\ensuremath{\ma{F}}}
\newcommand{\Fmax}{\ensuremath{\Fm^*}\xspace}
\newcommand{\Fma}{$\ma{F}_{\ma{A}}$\xspace}

\def\eve#1{\textbf{\em #1}}
\newcommand{\ve}[1][x]{\ensuremath{\mathbf{#1}}\xspace}
\newcommand\twid[1][x]{\stackrel{\sim}{\smash{#1}\rule{0pt}{1.1ex}}}
\newcommand\vtwid[1][x]{\stackrel{\sim}{\smash{\ve[#1]}\rule{0pt}{1.1ex}}}

\newcommand{\linf}{\ensuremath{\ve[l_{\infty}]}\xspace}
\newcommand{\estlinf}{\ensuremath{\ve[\hat{l}_{\infty}]}\xspace}
\newcommand{\A}{\ensuremath{\ma{A}}\xspace}
\newcommand{\estA}{\ensuremath{\ma{\hat{A}}}\xspace}

\newcount\colveccount
\newcommand*\colvec[1]{
        \global\colveccount#1
        \begin{pmatrix}
        \colvecnext
}
\def\colvecnext#1{
        #1
        \global\advance\colveccount-1
        \ifnum\colveccount>0
                \\
                \expandafter\colvecnext
        \else
                \end{pmatrix}
        \fi
}

\newtoks\rowvectoks
\newcommand{\rowvec}[2]{%
  \rowvectoks={#2}\count255=#1\relax
  \advance\count255 by -1
  \rowvecnexta}
\newcommand{\rowvecnexta}{%
  \ifnum\count255>0
    \expandafter\rowvecnextb
  \else
    \begin{pmatrix}\the\rowvectoks\end{pmatrix}
  \fi}
\newcommand\rowvecnextb[1]{%
    \rowvectoks=\expandafter{\the\rowvectoks&#1}%
    \advance\count255 by -1
    \rowvecnexta}

% symbols
\newcommand{\R}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\Ps}{\ensuremath{\mathbb{P}}\xspace}
\newcommand{\X}{\ensuremath{\mathbb{X}}\xspace}
\newcommand{\N}{\ensuremath{\mathbb{N}}\xspace}
%\newcommand{\see}[1]{(\ref{#1})\xspace}
\newcommand{\eps}{\ensuremath{\varepsilon}\xspace}
\newcommand{\I}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\IImax}{\ensuremath{\mathcal{I}^*}\xspace}

\newcommand{\mmm}{\ensuremath{\mathcal{m}}\xspace}
\newcommand{\ie}{{\em i.e.}\xspace}
\newcommand{\eg}{{\em e.g.}\xspace}
%\newcommand{\etc}{{\em etc.}\xspace}
\newcommand{\etal}{et al.}
\newcommand{\parsp}{\ensuremath{\Theta}\xspace}
\newcommand{\etan}{\ensuremath{\eta_{_0}}\xspace}
\newcommand{\thr}{\ensuremath{\Delta}\xspace}
\newcommand{\cbd}{\hfill \ensuremath{\Box} \\}
\newcommand{\T}{{\!\top}}
%\newcommand{\mT}{{-\!\top}}
%\newcommand{\proof}{\par \noindent {\em Proof:}\ }
%\newcommand{\note}{\par \noindent {\em Note:}\ }
%\newcommand{\nsim}{\not \sim}
\providecommand{\nsim}{\not \sim}
\newcommand{\ssym}[1]{[#1]_{\times}}
\newcommand{\set}[1]{\ensuremath{\mathcal{#1}}\xspace}
\renewcommand{\O}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\sam}{\set{M}}
\newcommand{\dpt}{\ensuremath{\mathbf u}\xspace}
\newcommand{\U}{\set{U}}
\newcommand{\supp}{\set{S}}

\newcommand{\Imax}{\ensuremath{I^*}\xspace}
\newcommand{\opt}[1]{\ensuremath{#1^*}\xspace}
\newcommand{\Umax}{\ensuremath{U^*}\xspace}

\def\oversim#1#2{\lower .5pt\vbox{\lineskiplimit=\maxdimen \lineskip=.5pt
    \ialign{$\mathsurround=0pt #1\hfil ##\hfil $\crcr #2\crcr \sim\crcr }}}
\def\simplus{\mathrel{\mathpalette\oversim{\scriptscriptstyle+}}}

\newcommand{\bad}{``bad''\xspace}
\newcommand{\good}{``good''\xspace}

%R-RANSAC
\newcommand{\Hgs}{\ensuremath{H_g}\xspace}
\newcommand{\Hws}{\ensuremath{H_b}\xspace}
\newcommand{\Pgs}{\ensuremath{P_{g}}\xspace}
\newcommand{\tM}{\ensuremath{t_{M}}\xspace}
\newcommand{\tV}{\ensuremath{t_{V}}\xspace}
\newcommand{\ms}{\ensuremath{\overline{m}_S}\xspace}

\newcommand{\cluster}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\motif}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\repetition}{\ensuremath{\mathcal{R}}\xspace}
\newcommand{\dist}{\ensuremath{\mathcal{L}_{\lambda}}\xspace}
\newcommand{\udist}{\ensuremath{\mathcal{L}^\inv_{\lambda}}\xspace}

\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}

% alignment
\newcommand{\pairbox}[3][.45\linewidth]{\mbox{} \hfill
    \parbox[t]{#1}{\centering #2} \hfill \parbox[t]{#1}{\centering #3} \hfill \mbox{}}

\newcommand{\tribox}[4][.3\linewidth]{\mbox{} \hfill
    \parbox[t]{#1}{\centering #2} \hfill \parbox[t]{#1}{\centering #3} \hfill
    \parbox[t]{#1}{\centering #4} \hfill \mbox{}}

% ALGORITHM
\newfloat{algorithm}{tbh}{loa}
\floatname{algorithm}{Algorithm}
\let \oldalgortihm = \algorithm
\def \algorithm {\oldalgortihm \noindent \hbox{} \hrulefill
\\[-12pt]
\let \oldcaption = \caption
\def \caption {\mbox{}\\[-15pt] \noindent \hbox{} \hrulefill \oldcaption}}

% THEOREMS
%\newtheorem{experiment}{Experiment}
%\newtheorem{definition}{Definition}
%\newtheorem{theorem}{Theorem}
%\newtheorem{proposition}{Proposition}
%\newtheorem{example}{Example}
%\newtheorem{result}{Result}
%\newtheorem{assumption}{Assumption}

% references
\newcommand{\eq}[1]{Eq.~{#1}}
\newcommand{\fig}[1]{Fig.~{#1}}
\newcommand{\figs}[1]{Figs.~{#1}}

\newcommand{\tab}[1]{Tab.~{#1}}
\newcommand{\alg}[1]{Alg.~{#1}}
\newcommand{\secref}[1]{section~{#1}}
\newcommand{\Secref}[1]{Section~{#1}}
\newcommand{\chapref}[1]{{chapter~\ref{#1}}\xspace}
\newcommand{\appref}[1]{appendix~{#1}}


%others
\newcommand{\thesis}{thesis\xspace}

\definecolor{faded}{rgb}{.97,.97,.97}
\newcommand{\confidentialscale}{4.2}
\newcommand{\confidential}[1]{
\watermark{\begin{minipage}[t]{.99\linewidth}
\mbox{}\\[-1cm]
{\footnotesize \mbox{#1}\\}
\rotatebox{-64}{\scalebox{\confidentialscale}{\Huge \color{faded}{CONFIDENTIAL}}}
\end{minipage}}} 

\makeatletter
\newcommand*{\pmzeroslash}{%
  \nfss@text{%
    \sbox0{0}%
    \sbox2{/}%
    \sbox4{%
      \raise\dimexpr((\ht0-\dp0)-(\ht2-\dp2))/2\relax\copy2 %
    }%
    \ooalign{%
      \hfill\copy4 \hfill\cr
      \hfill0\hfill\cr
    }%
    \vphantom{0\copy4 }% correct overall height and depth of the
                       % symbol
  }%
}
\makeatother


\endinput


==> tables.tex <==
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Metric & Method & Repeats & Groups & Planes & Linfs\tabularnewline
\hline
\hline
\multirow{3}{*}{W-miavF} & Proposed & \textbf{0.42} & \textbf{0.61} & \textbf{0.62} & \textbf{0.73}\tabularnewline
\cline{2-6}
& MultiRANSAC & 0.30 & 0.41 & 0.41 & 0.56\tabularnewline
\cline{2-6}
& J-Linkage & 0.40 & 0.57 & 0.58 & 0.65\tabularnewline
\hline
\multirow{3}{*}{NW-maavF} & Proposed & \textbf{0.34} & \textbf{0.46} & \textbf{0.53} & \textbf{0.62}\tabularnewline
\cline{2-6}
& MultiRANSAC & 0.19 & 0.27 & 0.33 & 0.40\tabularnewline
\cline{2-6}
& J-Linkage & 0.33 & 0.45 & 0.52 & 0.50\tabularnewline
\hline
\multirow{3}{*}{AMI} & Proposed & \textbf{NaN} & \textbf{NaN} & \textbf{NaN} & \textbf{NaN}\tabularnewline
\cline{2-6}
& MultiRANSAC & NaN & NaN & NaN & NaN\tabularnewline
\cline{2-6}
& J-Linkage & NaN & NaN & NaN & NaN\tabularnewline
\hline
\multirow{3}{*}{Affine} & Proposed & \textbf{} & \textbf{} & \textbf{} & \textbf{3.84}\tabularnewline
\cline{2-6}
& MultiRANSAC &  &  &  & 7.03\tabularnewline
\cline{2-6}
& J-Linkage &  &  &  & 8.25\tabularnewline
\hline
\end{tabular}
\par\end{center}


